Who Will Support My Project? Interactive Search of Potential Crowdfunding Investors Through InSearch

Crowdfunding provides project founders with a convenient way to reach online investors. However, it is challenging for founders to find the most potential investors and successfully raise money for their projects on crowdfunding platforms. A few machine learning based methods have been proposed to recommend investors' interest in a specific crowdfunding project, but they fail to provide project founders with explanations in detail for these recommendations, thereby leading to an erosion of trust in predicted investors. To help crowdfunding founders find truly interested investors, we conducted semi-structured interviews with four crowdfunding experts and presents inSearch, a visual analytic system. inSearch allows founders to search for investors interactively on crowdfunding platforms. It supports an effective overview of potential investors by leveraging a Graph Neural Network to model investor preferences. Besides, it enables interactive exploration and comparison of the temporal evolution of different investors' investment details.

==> panel_study.tex <==
\section{Background}
\label{sec:background}




% 
% \subsection{Kickstarter}\label{sec:Kickstarter}
% \subsection{kickstarter}
There are two sections to our background: dataset preparation and the analysis required to obtain prospective investors.

% \yong{Songheng, backers or investors? Please use only one term throughout the paper.}

\subsection{Dataset}
There are many crowdfunding platforms where project founders can initiate projects to obtain capital from the platform users. Kickstart, a crowdfunding platform that focuses on rewarding projects, has emerged from these platforms and is making a significant impact in the field. Kickstarter has successfully raised 6 billion dollars ~\cite{kickstarter}. In this article, we collect crowdfunding-related data from Kickstarter. The dataset contains 41277 projects launched on Kickstarter and 762 investors who have invested in these projects. 

The project features include:
\begin{itemize}
  \item \textbf{Goal}: The founders hope to raise funds for the corresponding projects.
  \item \textbf{Category}: Hierarchical category of projects. The category data includes 15 main categories and 161 subcategories.
  \item \textbf{Updates}: Short blog post aims to inform investors about the project status.
  \item \textbf{Story}: Textual description introduces a project.
  \item \textbf{Comments}: Comment frequency records the level of investor participation in a project.
  \item \textbf{Launching Time}: The year-month timestamp indicates when a project starts.
\end{itemize}

Additionally, an investor's features include:
\begin{itemize}
    \item \textbf{Investment Number}: The number of projects this investor has invested in.
    \item \textbf{Location}: It refers to the location shown on an investor's profile.
\end{itemize}

%我们对数据做了什么处理,有什么工作支撑我们的feature selection.
The target goal size of the project is crucial to its success.~\cite{ferreira2018success}~\cite{yu2018prediction}. A project's success rate varies depending on its category. Games and design are the most likely to succeed~\cite{jankuu2018successful}. Project updates are used to keep Kickstarter investors informed of the specific progress~\cite{Kickstarterfaq}.  
The quality of the update has a significant impact on investors' decision to invest~\cite{xu2014show}. Textual description of the project, comments, and launching time is an important predictor of the Kickstarter project success~\cite{mitra2014language}~\cite{ryoba2020right}~\cite{stanislovaitis_2019}. Besides, investors' investment numbers are essential in Kickstarter. Investors who invest in 25 projects or more are called "super supporters," and their presence is important to campaign founders~\cite{stanislovaitis_2019}. Additionally, the match between an investor and a project launch location is crucial~\cite{rakesh2015project}.

In data prepossessing, we have divided the project goal amount into four intervals based on size: 0-1000, 1000-1000,10000-25000,25000 to more. In the model, project categories are classified according to their subcategories. The location of investors and projects is assigned based on their country of origin if the origin is outside the United States. Otherwise, the location is assigned according to the United States and specific states. And in the interaction system, to prevent information overload, we refer to Indegogo (another popular crowdfunding platform, similar to Kickstarter) and redefine the 15 categories into four categories (Games, Arts, Publishing \& Writing, Technology \& Innovation).



% 关于requirement  analysis的写作，你可以找几篇vast文章参考下写作思路，基本上都是
% 1. 先说大致怎么得到这些requirements：interview或者调研相关文献
% 2. 然后分别介绍每个requirement，并说明细节理由。如果可以的话，你也可以考虑把这些requirements分成不同的层级或者group

% if have more time, refer to Dfseer to write more details in design view collections
\subsection{Requirement Analysis}
In this paper, we worked closely with four crowdfunding domain experts and gathered valuable suggestions for the system design. One expert is the CEO of a crowdfunding agency that has helped founders of projects raise tens of millions of dollars. Another expert is the author of a popular handbook for crowdfunding founders and has participated in some crowdfunding projects. The other two experts have launched several crowdfunding projects.

In this paper, we worked closely with four crowdfunding domain experts and gathered valuable suggestions for the system design. One expert is the CEO of a crowdfunding agency that has helped founders raise tens of millions of dollars. Another expert is the author of a popular handbook for crowdfunding founders and has participated in some crowdfunding projects. The other two experts have launched several crowdfunding projects.

%embedding view
\textbf{R1. Filter out prospective investors who are interested in the founders' project.} Based on some user-defined project characteristics, the system should automatically recommend a set of interested investors. Additionally, the user should be able to select similar investors in clusters manually. 

%timeline chart
\textbf{R2. Identify several investors' long-term investment preferences quickly.} Using the system, a user can identify the selected investors' long-term preferences and investment frequency, which helps the user to detect investment patterns. In addition, the system allows the user to select a time interval, and then further scrutinize the investment details that occurred in that time period. In a time interval, the system will display an overview of selected investors' particular investment preferences

%treemap
\textbf{R3. Give an overview of an investor's investment portfolio.} In addition to the overviews of funded projects by selected investors, the system should also display the characteristics distribution of funded projects from one particular investor, either by project category or by project size.

%textflow, and bar glyph
\textbf{R4. Analyzing characteristics of investors' funded projects.} When analyzing an investor's decision patterns, a user should also be aware of the characteristics of projects in detail. Therefore, the system enables users to analyze corresponding projects’ important attributes.

\textbf{R5. intuitively discover investors with similar preferences.} A user can straightforwardly get the similarity of investors by their positions on the 2D space. Then a user can quickly get an overview of investors by selecting them.


% from expert
% from reading book and article


